Learning in Quantum Common-Interest Games and the Separability Problem

Learning in games has emerged as a powerful tool for machine learning with numerous applications. Quantum games model interactions between strategic players who have access to quantum resources, and several recent works have studied {learning in} the competitive regime of quantum zero-sum games. Going beyond this setting, we introduce quantum common-interest games (CIGs) where players have density matrices as strategies and their interests are perfectly aligned. We bridge the gap between optimization and game theory by establishing the equivalence between KKT (first-order stationary) points of an instance of the Best Separable State (BSS) problem and the Nash equilibria of its corresponding quantum CIG. This allows learning dynamics for the quantum CIG to be seen as decentralized algorithms for the BSS problem. Taking the perspective of learning in games, we then introduce non-commutative extensions of the continuous-time replicator dynamics and the discrete-time best response dynamics/linear multiplicative weights update for learning in quantum CIGs. We prove analogues of classical convergence results of the dynamics and explore differences which arise in the quantum setting. Finally, we corroborate our theoretical findings through extensive experiments.

==> preamble_quantum.tex <==
\usepackage[utf8]{inputenc}

%% Sets page size and margins
%\usepackage[a4paper,top=3cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=2cm]{geometry}
% \usepackage{geometry}
% \usepackage[verbose=true,letterpaper]{geometry}
% \AtBeginDocument{
%   \newgeometry{
%     textheight=9in,
%     textwidth=5.5in,
%     top=1in,
%     headheight=12pt,
%     headsep=25pt,
%     footskip=30pt
%   }
%   \@ifpackageloaded{fullpage}
%     {\PackageWarning{neurips_2022}{fullpage package not allowed! Overwriting formatting.}}
%     {}
% }
%% Math
\usepackage{amsmath,amsfonts,amssymb, amsthm}
%% Paragraph formatting
\usepackage[parfill]{parskip}
%% Enum labels
\usepackage[shortlabels]{enumitem}
%% Hyperlink References
% \usepackage[colorlinks=true, allcolors=blue]{hyperref}
%% AMS symb, for \mathbb
\usepackage{amssymb}
%% physics package, for derivatives
\usepackage{physics}
\usepackage{braket}
%% sfrac slanted fractions in powers
\usepackage{xfrac}
%% captions
\usepackage[singlelinecheck = false]{caption}

% \captionsetup[algorithmic]{labelformat=empty}
%% Placing image "right here"
\usepackage{float}
\usepackage{graphicx}
\usepackage[justification=centering]{caption}
%subfigures
\usepackage{subcaption}
% strikethrough
\usepackage{soul}
\usepackage{cancel} %diagonal strikethroughs \cancel
% Colors
\usepackage{xcolor}
%subequations, braces
\usepackage[overload]{empheq} 
% fullcite
%\usepackage[style=authoryear]{biblatex}
%\addbibresource{ref.bib}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{algorithmic}
% Divergence
\usepackage{mathtools}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{D\infdivx}




%%Argmin, Argmax
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

%%% Antonios new commands
\newcommand{\sfT}{{\sf T}}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\bbS}{\mathbb{S}}
\def\bal{\begin{aligned}}
\def\eal{\end{aligned}}
\newcommand{\psd}{\mathbb{S}_+}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\p}{\partial}
\newcommand{\sub}{\subseteq}
\newcommand{\lam}{\lambda}
\newcommand{\calf}{\mathcal{F}}
\newcommand{\face}{\triangleleft}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\amin}{\mathrm{argmin}}
\DeclareMathOperator{\dee}{d}
\DeclareMathOperator{\vect}{vec}
\DeclareMathOperator{\sgn}{sgn}



\DeclareMathOperator{\cala}{\mathcal{A}}



\def\be{\begin{equation}}
\def\ee{\end{equation}}



\newcommand{\mca}{\mathcal{A}}
\newcommand{\mcb}{\mathcal{B}}

\newcommand{\mcx}{\mathcal{X}}
\newcommand{\mcs}{\mathcal{S}}

%%% Wayne new commands
%% Lines
\newcommand*\linetiny[0]{\vspace{6pt}}
\newcommand*\linesmall[0]{\vspace{12pt}}
\newcommand*\linemed[0]{\vspace{18pt}}
\newcommand*\linelarge[0]{\vspace{24pt}}
%% Math
\newcommand*\vectorize[1]{\mathrm{vec}(#1)}
\newcommand*\innerprod[2]{\left\langle #1, #2 \right\rangle}
\newcommand*\transpose[1]{{#1}^\top}
\newcommand*\inv[1]{{#1}^{-1}}
% Spaces
\newcommand*\matspace[1]{\mathbb{M}_{#1}}
\newcommand*\symmmatspace[1]{\mathbb{S}^{#1}}
\newcommand*\rnonneg[0]{\mathbb{R}_{+}}
% Opti problems
\newcommand*\optispace[0]{\;}
\newcommand*\minimize[1]{\min_{#1} \optispace}
% Equality
\newcommand*\equalslong[0]{\quad = \quad}
%% new and old
\newcommand*\new[1]{{#1}^{new}}
\newcommand*\old[1]{{#1}^{old}}
%% qualifiers
\newcommand*\fa[0]{ \forall \;}
\newcommand*\sfa[0]{\;\, \fa}
%% Sets
\newcommand*\ortho[1]{\mathcal{O}_{#1}}
\newcommand*\simplex[1]{\triangle_{#1-1}}
\newcommand*\conv[1]{\mathrm{conv}\left(#1\right)}
\newcommand*\verts[0]{\; \vert \;}
\newcommand*\diag[1]{\mathrm{diag}\left(#1\right)}
% PSD/PD cone
\newcommand*\psdcone[1]{\mathcal{S}^{#1}_{+}}
\newcommand*\pdcone[1]{\mathcal{S}^{#1}_{++}}
% Trace
\newcommand*\trac[1]{\Tr\left(#1\right)}
\newcommand*\tracsq[1]{\Tr\left[#1\right]}
% Power half and negative-half
\newcommand*\powh[1]{#1^{\sfrac{1}{2}}}
\newcommand*\pownh[1]{#1^{-\sfrac{1}{2}}}
% Online Combinatorial Opti notation
\newcommand*\Dwish[2]{\mathcal{{#1}}{{#2}}}

%PSD rank
\newcommand*\psdrank[1]{\rank_{\text{psd}}\left(#1\right)}

%puri
\newcommand*\lps[1]{\text{LPS}_{\mathbb{#1}}}
\newcommand*\purirank[1]{\text{puri-rank}_{\mathbb{#1}}}

%Bregman Divergence, KL div
\newcommand*\bregdiv[3]{\mathrm{D}_{#1} \left(#2, \, #3 \right)}
\newcommand*\KLdiv[2]{\bregdiv{\text{KL}}{#1}{#2}}

%Component-wise product
\newcommand*\compprod[0]{\circ}

%Vectorized function
\newcommand*\vecf[1]{\underline{#1}}
\newcommand*\matvec[1]{\mathbf{#1}}
\newcommand*\matf[1]{\mathbf{#1}}

%scaled squares and circles
\usepackage{scalerel}
\def\mcirc{\mathbin{\scalerel*{\circ}{j}}}
\def\msquare{\mathord{\scalerel*{\Box}{gX}}}

% theorem-like environments
\newtheorem{definition}{Definition}[section]
\newtheorem*{definition*}{Definition}
\newtheorem{lemma}{Lemma}[section]
\newtheorem*{lemma*}{Lemma}
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{corollary}{Corollary}[section]
\newtheorem*{corollary*}{Corollary}
\theoremstyle{plain}
\newtheorem{informaltheorem}{Informal Theorem}[section]


%% Figures
\usepackage{graphicx}
\usepackage{caption}
% \newenvironment{Figure}
%   {\par\medskip\noindent\minipage{\linewidth}}
%   {\endminipage\par\medskip}
% \usepackage[font={small,it}]{caption}
% \usepackage[justification=centering]{caption}


%Adjoint, Hermitian conjugate
\newcommand*\adj[1]{{#1}^*}
\newcommand*\hermconj[1]{{#1}^\dagger}

%%To copy in

%% Specific notation
\newcommand*\Herm[1]{H^{#1}}
\newcommand*\HermPSD[1]{\Herm{#1}_+}
\newcommand*\HermPD[1]{\Herm{#1}_{++}}
\newcommand*\density[1]{D^{#1}}
% \newcommand*\adj[1]{{#1}^\dagger}

\newcommand*\opt[1]{\mathrm{OPT}(#1)}
\newcommand*\subj[0]{\mathrm{subject\,to}\quad}

\newcommand*\field[0]{\mathbb{F}}


%% Probability & Statistics
\newcommand*\prob[1]{\mathbb{P}\left[{#1}\right]}
\newcommand*\probp[1]{\mathbb{P}\left({#1}\right)}
\newcommand*\expect[0]{\mathop{\mathbb{E}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

%% Game Theory
\newcommand*\stratprofspace[0]{\mathbf{S}}
\newcommand*\stratspace[1]{S_{#1}}
\newcommand*\stratprof[0]{\mathbf{s}}
\newcommand*\strat[1]{s_{#1}}
\newcommand*\payoffvec[0]{\mathbf{u}}
\newcommand*\payoffto[1]{u_{#1}}
\newcommand*\given[0]{\, \vert \,}

%% Complex numbers
%\newcommand*\conj[1]{\overline{#1}}

% Linear Algebra
\newcommand*\vsp[1]{\mathcal{#1}}
\newcommand*\linmaps[2]{L(\vsp{#1}, \vsp{#2})}
\newcommand*\linops[1]{L(\vsp{#1})}
\newcommand*\range[1]{\mathop{R}(#1)}

% Sectioning
\newcommand*\bundl[1]{\textbf{\underline{#1}}}

% Information theory
\newcommand*\relent[2]{\mathbf{S}\left(#1 || #2 \right)}

% Functions
\newcommand*\dom[0]{\mathop{dom}}

%%% Paper-Specific
% EigenGame PCA
\newcommand*\hv[0]{\hat{v}}

%%%Topology
\newcommand*\inte[1]{\mathrm{int}(#1)}

%%% Theorem formatting
% \theoremstyle{plain}
\newtheorem{thm}{Theorem}[section] % reset theorem numbering for each section
\newtheorem{lem}[thm]{Lemma} % same for lemma numbers
% \theoremstyle{definition}
\newtheorem{defn}[thm]{Definition} % definition numbers are dependent on theorem numbers
%\newtheorem{thm}{Theorem}
%\newtheorem{defn}{Definition}
% \newtheorem{observation}{Observation}[section]
\newtheorem{question}{Question}[section]
% \newtheorem{claim}{Claim}[section]
\newtheorem{fact}{Fact}[section]
\newtheorem{assumption}{Assumption}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{example}{Example}[section]
\newtheorem{remark}{Remark}[section]

% ditto marks
\usepackage[T1]{fontenc}
%\newcommand*{\ditto}{\mbox{---} \textquotedbl \mbox{---}}
\newcommand*{\ditto}{\mbox{---} \texttt{"} \mbox{---}}

% Game Theory
\newcommand*\playerset[0]{{N}}
\newcommand*\playernum[0]{\abs{\playerset}}
\newcommand*\payoff[1]{u_{#1}}
\newcommand*\strategyset[1]{\mathcal{A}_{#1}}

%% Sets (EJAs)
\newcommand{\R}[0]{\mathbb{R}}
\newcommand{\C}[0]{\mathbb{C}}
\newcommand{\Q}[0]{\mathbb{Q}}
%
\newcommand{\A}[0]{\mathcal{A}}
\newcommand{\B}[0]{\mathcal{B}}
\newcommand{\K}[0]{\mathcal{K}}
\newcommand{\I}[0]{\mathcal{I}}
\newcommand{\V}[0]{\mathbb{V}}
\renewcommand{\H}[0]{\mathcal{H}}

%
\newcommand{\Sym}[0]{\mathbb{S}}
%
\newcommand{\HermJ}[0]{\mathrm{Herm}}
\renewcommand*{\Herm}[0]{\mathbb{H}}

\newcommand*{\SOC}[0]{\mathcal{Q}}
\newcommand*{\JSA}[0]{\mathbb{L}}

% To do list (with checkboxes)
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}%
\hspace{-2.5pt}}
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}}
\newcommand{\prio}{\rlap{$\square$}{\raisebox{1pt}{\large$\color{red}{\bigcirc}$}}}%
%add-ons?
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,scale=.8,inner sep=1pt] (char) {#1};}}

%one vector
\newcommand*{\one}{\mathbf{1}}

%eigenvalues
\newcommand*\lmin[0]{\mathrm{\lambda_{\min}}}
\newcommand*\lmax[0]{\mathrm{\lambda_{\max}}}

%Divergence
\newcommand*\Di[2]{\mathrm{D}(#1 \, \vert \vert \, #2)}


%conjugation
\newcommand*\conj[2]{\powh{#1} #2 \powh{#1}}


%distance
\newcommand*\D[0]{\mathop{D}}


\newcommand{\timesx}{S_1\times \ldots \times S_k}
\newcommand{\prodsim}{\Delta(\times_{i=1}^k S_i)}

\def \bbb{\color{blue}}
\def \kkk{\color{black}}
\def \rrr{\color{red}}
\def \fff{\color{gray}}

% \newcommand{\Tr}{\mathrm{Tr}}
% \newcommand{\id}{\mathbb{1}}
% \newcommand{\ket}[1]{\vert {#1} \rangle}
% \newcommand{\bra}[1]{\langle {#1} \vert}
% \newcommand{\braket}[2]{\langle {#1} \vert {#2} \rangle}
% \DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
% \setcitestyle{square}
% \hypersetup{
%     colorlinks=true,
%     linkcolor = black,
%     urlcolor=blue,
%     citecolor=black
% }

\newcommand*\da{\mathrm{D}(\mathcal{A})}
\newcommand*\db{\mathrm{D}(\mathcal{B})}

\newcommand*\id{\mathbb{I}}
